Associated Permutations of Complete Non-Ambiguous Trees

We explore new connections between complete non-ambiguous trees (CNATs) and permutations. We give a bijection between tree-like tableaux and a specific subset of CNATs. This map is used to establish and solve a recurrence relation for the number of tree-like tableaux of a fixed size without occupied corners, proving a conjecture by Laborde-Zubieta. We end by establishing a row/column swapping operation on CNATs and identify new areas for future research.

==> preamble.tex <==



%Packages
\usepackage[a4paper, margin=1in]{geometry}
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{amsfonts} 
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{hyperref}
\usepackage{verbatim}
\usepackage{mdframed}
\usepackage{xcolor}
\usepackage{changepage}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{pst-node}
\usepackage{auto-pst-pdf}
\usepackage{array}
\usepackage{nicematrix}
\usepackage{float}
\usepackage{thmtools, thm-restate}
\usepackage[capitalize]{cleveref}
\usepackage{ytableau}
\usepackage{diagbox}
\usepackage{authblk}

\graphicspath{ {./figures/} }

%Custom commands
\newcommand{\Nn}{\mathbb{N}}
\newcommand{\Rr}{\mathbb{R}}
\newcommand{\Qq}{\mathbb{Q}}
\newcommand{\Zz}{\mathbb{Z}}
\newcommand{\Hy}{\mathbb{H}}
\newcommand{\sgn}{\text{sgn}}



\setlength{\parindent}{1em}
\setlength{\parskip}{1em}



%Theorem styles
\newtheorem{thm}{Theorem}
\newtheorem{conj}[thm]{Conjecture}


\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{rem}[thm]{Remark}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{example}[thm]{Example}

\numberwithin{thm}{section}
\numberwithin{defn}{section}

\numberwithin{rem}{section}
\numberwithin{conj}{section}
\numberwithin{lem}{section}
\numberwithin{cor}{section}
\numberwithin{example}{section}
\numberwithin{prop}{section}
\numberwithin{figure}{section}

\allowdisplaybreaks
